A framework for implementing general virtual element spaces

In this paper we present a framework for the construction and implementation of general virtual element spaces based on projections built from constrained least squares problems. Building on the triples used for finite element spaces, we introduce the concept of a VEM tuple which encodes the necessary building blocks to construct these projections. Using this approach, a wide range of virtual element spaces can be defined. We discuss $H^k$-conforming spaces for $k=1,2$ as well as divergence and curl free spaces. This general framework has the advantage of being easily integrated into any existing finite element package and we demonstrate this within the open source software package DUNE.

==> Sections/acknowledgements.tex <==
\section*{Acknowledgements}

==> Sections/tikzdofs.tex <==
\begin{figure}[!h]
    \centering
    \begin{tikzpicture}
    %triangle 1:
        \draw (0,0) -- (2,0);
        \draw (0,0) -- (1,1.73);
        \draw (1,1.73) -- (2,0);

        \fill[black] (0,0) circle (0.075cm);
        \fill[black] (1,1.73) circle (0.075cm);
        \fill[black] (2,0) circle (0.075cm);

        \node at (1.85,0.87) {$e_{i}$};
        \node at (1,-0.25) {$e_{i-1}$};

        % \draw[arrows=->,line width=.4pt] (1,0) -- (1,-0.5);
        % \draw[arrows=->,line width=.4pt] (0.5,0.87) -- (0.067,1.12);

        \node at (-0.25,-0.25) {$v_{i-1}$};
        \node at (2.25,-0.25) {$v_{i}$};

        \node at (1,0.7) {$\element$};
    \end{tikzpicture}
    \caption{}
    \label{figure:}
\end{figure}
